MPD physics performance studies in Bi+Bi collisions at $\sqrt{s_{NN}}=9.2$ GeV

The Multi-Purpose Detector (MPD) is one of the three experiments of the Nuclotron Ion Collider-fAcility (NICA) complex, which is currently under construction at the Joint Institute for Nuclear Research in Dubna. With collisions of heavy ions in the collider mode, the MPD will cover the energy range 4-11 GeV to scan the high baryon-density region of the QCD phase diagram. With expected statistics of 50-100 million events collected during the first run, MPD will be able to study a number of observables, including measurements of light hadrons and hypernuclei production, particle flow, correlations and fluctuations, have a first look at dielectron production, and modification of vector-meson properties in dense matter. In this paper, we present selected results of the physics feasibility studies for the MPD experiment in Bismuth-Bismuth collisions at an energy of 9.2 GeV, the system considered as one of the first available at the NICA collider.

==> Levy_analysis.tex <==
\begin{figure*}
\centering
\begin{multicols}{2}
    \includegraphics[width=0.475\textwidth]{C2CRAB_fits_separation_levy_58.png}\par 
    \includegraphics[width=0.475\textwidth]{C2CRAB_fits_separation_smearing_58.png}\par 
    \end{multicols}
\caption{Two-pion correlation function of primary and secondary pions, produced in Bi+Bi collisions at $\sqrt{s_{NN}} = 5.8$ GeV, with impact parameter $b = 0-1$ fm. Solid lines represent the fit of L\'evy forms. Left panel shows the \textit{ideal resolution} case and the panel on the right shows the \textit{finite resolution} case with a $\Delta_q=10$ MeV smearing.}
\label{fig:C2-separation}
\end{figure*}



\begin{figure*}
\centering
\begin{multicols}{2}
    \includegraphics[width=\linewidth]{Rinv_IR_sNN.png}\par 
    \includegraphics[width=\linewidth]{Rinv_FR_sNN.png}\par 
    \end{multicols}
\begin{multicols}{2}
    \includegraphics[width=\linewidth]{alpha_IR_sNN.png}\par
    \includegraphics[width=\linewidth]{alpha_FR_sNN.png}\par
\end{multicols}
\caption{Source size $R_\text{inv}$ and L\'evy index of stability $\alpha$, as functions of the collision energy $\sqrt{s_{NN}}$, for the complete set of pions (black circles), primary pions (red rectangles) and secondary pions (blue diamonds), obtained from Bi+Bi collisions with impact parameter $b = 0-1$ fm. $R_\text{inv}$ and $\alpha$ are obtained from fits to a L\'evy form. Left column shows the \textit{ideal resolution} case and the right column shows the \textit{finite resolution} case with a $\Delta_q=10$ MeV smearing.}
\label{fig:RandA}
\end{figure*}


The two-pion correlation function is typically described by parameters that provide insight into both the space-time dimensions of the pion-emitting source and the mechanisms driving pion production. These parameters include the average source size, $R$, and the correlation strength, $\lambda$, which is the intercept at vanishing relative momentum. Given the dependence of particle production processes on collision energy, these parameters are expected to evolve accordingly. Identifying variations in these parameters, particularly within the NICA energy range, is important for exploring potential signals of criticality, such as the Critical End Point (CEP). As such, femtoscopic studies are a valuable tool for probing the QCD phase diagram~\cite{Csanad:2020xbf,Bzdak:2019pkr}. 

When the correlation function is described as a function of relative pair momentum for a fixed average pair momentum, it is commonly parametrized using a Gaussian function, based on the fact that the Fourier transform of a Gaussian is also Gaussian. However, recent work has shown that this assumption is often inadequate. A more accurate description can be achieved using a symmetric Lévy distribution~\cite{Cimerman:2019hva,Nagy:2023zbg,Csorgo:2003uv}, which accounts for sources with extended tails in configuration space. The Lévy distribution generalizes the Gaussian, where the exponent $\alpha$ (the Lévy index) ranges from $\alpha = 2$ for a Gaussian to $\alpha = 1$ for a Cauchy distribution. 

 Lévy-based two-pion correlation studies have been applied to experimental data, primarily at high-energy collisions such as SPS~\cite{Porfy:2023yii}, RHIC~\cite{Kincses:2016jsr}, and LHC~\cite{CMS:2023xyd}. Recent studies within the NICA energy range have been performed using MC-generated data for Bi+Bi collisions in Ref.~\cite{Ayala:2023sbb}, covering energies relevant to the MPD experiment: $\sqrt{s_{NN}} = 4.0$, 5.8, 7.7 and 9.2 GeV. These studies serve as a benchmark for future work that incorporates an Equation of State (EoS) and considers possible phase transitions. 

 By fitting MC data to a Lévy distribution, source parameters such as $R$, $\lambda$ and $\alpha$ are extracted for different collision energies. A distinction between pions from primary (direct) and secondary (decay) processes shows that primary pions arise from a smaller source, while secondary pions originate from a larger source. Furthermore, momentum smearing effects, which simulate finite momentum resolution in detectors, reveal that the core-halo picture can identify $\lambda$ with the square of the fraction of core pions~\cite{Wiedemann:1996ig,PHENIX:2017ino}. For the NICA energy range, the core still contains a notable fraction of pions from long-lived resonances, rather than being dominated by primary particles. Future MC studies incorporating an EoS may help identify changes in pion production processes that could indicate critical behavior. A one-dimensional analysis in terms of $q_{\text{inv}}$ is employed to simplify the study of non-Gaussian structures in the correlation function~\cite{PHENIX:2017ino}. 

If the relative momentum between the particles is much smaller than the average pair momentum, then the two-pion correlation as a function of $q_{\mbox{\small{inv}}}$ for a fixed average pair momentum $K$, can be written as~\cite{Wiedemann:1999qn,NA61SHINE:2023qzr}
\begin{equation}
    C_2(q_{\text{inv}},K) = 1+\frac{\left\vert \Tilde{S}(q_\text{inv},K)\right\vert^2}{\left\vert\Tilde{S}(0,K)\right\vert^2} ,
\end{equation}
where $\Tilde{S}$ is the Fourier transform of $S$, the source function. Since the simulations require a large amount of events to produce a statistically significant sample, hereby we consider all possible values of $K$ that contribute to a given $q_{\mbox{\small{inv}}}$, as an effective source that contains all possible length scales corresponding to all values of the pair momenta. 


 The two-pion correlation function can reach a maximum value of 2 at zero relative momentum, with the intercept denoted as $C_2 (q_{\mbox{\small{inv}}} \to 0) = 1 + \lambda$, where $\lambda$ is also known as the chaoticity or intercept parameter. However, effects such as final state interactions and finite experimental resolution can prevent $\lambda$ from reaching 1. These effects are understood through the core-halo picture, where long-lived resonances produce a halo component that may not be fully resolved due to detector limitations. The emitting source can be modeled as $S = S_{\text{core}} + S_{\text{halo}}$, where the core consists of pions from primary processes. The Fourier transforms of the core and halo components are
\begin{eqnarray}
    N_{\text{core}} &=& \Tilde{S}_{\text{core}}(0), \\
    N_{\text{halo}} &=& \Tilde{S}_{\text{halo}}(0),
\end{eqnarray}
yielding $\Tilde{S}(0) = N_{\text{core}} + N_{\text{halo}}$. For resolvable momentum, $\Tilde{S}(q_{\text{inv}}) \simeq \Tilde{S}_{\text{core}}(q_{\text{inv}})$, and the correlation function becomes
\begin{equation}
    C_2 (q_{\text{inv}}) =1 + \left(\frac{N_{\text{core}}}{N_{\text{core}}+N_{\text{halo}}}\right)^2\!\frac{\left\vert\Tilde{S}_{\text{core}}(q_{\text{inv}})\right\vert^2}{\left\vert\Tilde{S}_{\text{core}}(0)\right\vert^2}.
\end{equation}
Thus, the intercept $\lambda$ can be expressed as
\begin{equation}
    \label{eq:lambda}
    \lambda = \left(\frac{N_{\text{core}}}{N_{\text{core}}+N_{\text{halo}}}\right)^2.
\end{equation}
For experimental or MC data, the two-pion correlation function is defined as
\begin{equation}
    C_2 (q) = \frac{\mathcal{N}_B}{\mathcal{N}_A} \frac{A(q)}{B(q)},
\end{equation}
where $A(q)$ is the relative momentum distribution of pions from the same event (containing quantum statistical effects), and $B(q)$ is from different events (without Bose-Einstein correlations). $\mathcal{N}_{A}$ and $\mathcal{N}_{B}$ are normalization factors~\cite{NA61SHINE:2023qzr,Zajc:1984vb}.


We use MC simulations from the Ultra-relativistic Quantum Molecular Dynamics Model (UrQMD)\cite{Bass:1998ca,Bleicher:1999xi} in cascade mode to generate relative momentum distributions for five million Bi+Bi central collisions at NICA energies ($\sqrt{s_{NN}} = 4.0$, 5.8, 7.7 and 9.2 GeV), with the simulation stopped at 200 fm. Since UrQMD does not include quantum statistical correlations\cite{Li:2012np,Ermakov:2017knq}, we apply the "correlation after-burner" (CRAB)~\cite{Pratt:1994uf} to account for these. CRAB calculates the quantum correlation by boosting pion pair momenta to the pair center-of-mass frame, symmetrizing the wave function, and expressing the result as a function of $q_{\mbox{\small{inv}}}$. For systems characterized by large fluctuations, the source function exhibits power-law tails, leading to a non-Gaussian, symmetric stable Lévy distribution. In this case, the correlation function is given by
\begin{equation}
    \label{eq:C2Levy}
    C_2 (q_{\text{inv}}) = 1 + \lambda \exp(-\vert q_{\text{inv}} R_{\text{inv}}\vert^\alpha),
\end{equation}
where $\alpha$ is the stability index, potentially related to the QCD correlation critical exponent~\cite{Csorgo:2008ayr,Csorgo:2004sr,Csorgo:2005it}. To examine the core and halo origins of pions, we simulate without detector smearing and separate primary from secondary pions using UrQMD’s parent process identification. Secondary pions mainly result from decays of resonances such as $\rho$, $\Delta$, $\omega$ and others~\cite{Bolz:1992hc}, which, although not all long-lived, are produced throughout the system lifetime.


To account for finite resolution effects, recall that it has been reported that the NICA-MPD will have a minimum momentum resolution of about 1.5 \% for particles with total momentum around 0.2 GeV~\cite{Maevskiy:2020ank}. Therefore, the relative momentum resolution of MPD will be of about $\Delta_q=10$ MeV. This effect can be included in our studies by fixing the smearing parameter of CRAB to 10 MeV. This means that the momentum $p$ of a given particle will be assigned
the same value, provided it lies in the range $p\pm \Delta_q/2$, which in turn can be translated into a limit for the minimum pair momentum resolution. This finite resolution translates into the fact that source components whose characteristic size is larger than $R\gtrsim 1/\Delta_q$, cannot be resolved~\cite{Csorgo:1994in} and we hereby refer to these as the halo. 


 Figure~\ref{fig:C2-separation} shows the two-pion correlation function for Bi+Bi collisions at $\sqrt{s_{NN}} = 5.8$ GeV with impact parameter $b = 0-1$ fm, together with the corresponding fits to a L\'evy form given by the solid lines. The left panel shows the separate contribution from primary and secondary pions to the the total correlation function in the \textit{ideal resolution case}. These results are consistent with the picture whereby primary pions come mainly from the core, since their source has a size significantly smaller than that of secondary pions. The panel on the right shows the \textit{finite resolution case} that includes a $\Delta_q=10$ MeV smearing on the separation of primary and secondary pions. 
 

 Figure~\ref{fig:RandA} shows the source size $R_\text{inv}$ and L\'evy index of stability $\alpha$, as functions of the collision energy $\sqrt{s_{NN}}$, for the complete set of pions, primary pions and secondary pions, obtained from Bi+Bi collisions with impact parameter $b = 0-1$ fm. $R_\text{inv}$ and $\alpha$ are obtained from fits to a L\'evy form. Left column shows the \textit{ideal resolution} case and the right column shows the \textit{finite resolution} case with a $\Delta_q=10$ MeV smearing.

 
For most of the studied energies the following hierarchy of source size parameters holds: $R_{\text{inv, prim}} < R_{\text{inv, all}} < R_{\text{inv, second}}$, except for the largest energy considered where we have instead $R_{\text{inv, prim}} <R_{\text{inv, second}}< R_{\text{inv, all}}$. This may seem somewhat confusing if one thinks that the larger portion of secondary pions should come from the halo, since they originate from long-lived resonances. The index $\alpha$ slightly decreases with the collision energy from the lowest to the largest energy considered but, except for the case of the primary pion sample, the overall decrease is non-monotonic. To summarize, for the perfect detector case, the general tendency for the source radii is to grow with the collision energy, while the L\'evy index of stability does not have a clear general tendency. The values of $R_{\text{inv}}$ for secondary pions are very similar but in general larger than those of the complete set of pions for the whole energy range; the opposite happens in general for the index $\alpha$.


 The finite resolution has the effect of diminishing the source size (by about 2\% for primary pions and about 21\%, for secondaries) and the value of the intercept (by about 8\% for primary pions and about 39\% for secondary pions), while the value of the L\'evy index decreases for primary pions (by about 8\%) and increases for secondary pions (by about 10\%). This means that the effect of the finite resolution is of the same order for the set containing all the pions than for the set containing only the secondary pions, while the effect of a finite resolution barely affects the set of primary pions.


 The results indicate that the core pion sample has a large component that comes from the decay of long-lived but slow-moving resonances, as well as a small component of pions coming from primary processes. The former decreases whereas the latter increases with collision energy. In this sense, the analysis of the relative abundance of pions in the core coming from resonance decays and from primary processes, as the collision energy changes, becomes more important as a tool to study signals of criticality within the NICA energy range.




==> factorial_moments.tex <==
One of the evidences of the phase transition is the increase of the power of multiplicity fluctuations~\cite{Hippert:2017xoj} which in turn means the change in the behavior of the moments of the multiplicity distribution in phase space intervals. However, one of the problems in studying moments is that dynamic fluctuations are obscured by statistical ones. The method to suppress statistical fluctuations by means of the use of the normalized factorial moments dependency on the interval size was proposed by A.~Bialas and R.~Peschanski~\cite{Bialas:1985jb}.
The dependence of the normalized factorial moments of the multiplicity distribution 
in bins over phase space on the bin size (intermittency) appears revealing dynamical 
fluctuations in the underlying process. Factorial moments were studied in Refs.~\cite{Antoniou:2014spa,MohisinKhan:2016huv} and the rise  of the factorial moments as a function of M was observed. Intermittency have been studied for heavy ion collisions by SHINE~\cite{Davis:2020fcy}. 
Recently, it was proposed to use this method to distinguish between different 
types of phase transition~\cite{NA49:2012ebu, Kodolova:2021yoh,Cheremnova:2022fsd}.



   Method of factorial moments uses the different normalization and averaging order for 
factorial moments which affect the dependence of the factorial moments on the bin size. 
If averaging is executed firstly over bins and then over events it is called horizontal. 
If ordering is changed and averaging is firstly done over events and then over bins, 
it is called vertical. Also normalization can be done on $<N(N-1)>$ or on $<N>$. -- DEFINE N --

The definition of the normalized factorial moments with horizontal averaging is more easy for interpretation as it gives $F_i(M=1)=1$, where M is the number of divisions of the initial interval:
\begin{equation}
  F_{i}(M) = M^{i-1} \times \frac{\sum_{j=1}^{M}{k_{j}\times(k_{j}-1)
  \times...\times(k_{j}-i+1)}}{N\times(N-1)\times...\times(N-i+1)},
\end{equation}
where $\delta y$, the bin size, 
$\delta y$ = $\Delta y/M$, $k_j$ is the number of particles in bin $j$, $N$ is the number 
of particles at the interval $\Delta y$, 
$i$ is the order of moment. In the case if fluctuations are purely statistical 
no variations of the $F_i$ as a function of $\delta y$ is expected while in the 
presence of the non-statistical fluctuations $F_i$ starts to increase with 
decreasing $\delta y$. However, the rise strongly depends on the underlying physics 
and the interpretation of the function behavior is not straightforward.
  Although there are a lot of attempts to connect the behaviour of the factorial moments 
with the fractal nature of particle collision~\cite{Bialas:1985jb},\cite{Sharma:2018vtf}-\cite{Sarma:2019teo} there exist also other reasons considered as short range correlations, Bose-Einstein correlations, resonances, phase transition, cascades, hadronization etc. From the experimental point of view clan model~\cite{Giovannini:1987tw} may appear easier for interpretation and connection with collision dynamics. 
Let's assume the simple mathematical model: random number of particles are organized in groups (clusters, sources) which are uniformly distributed along pseudorapidity interval.
The number of particles in group is accident. The case of each group to have 1 particle corresponds to the independent particle production. The additional considerations are that 
the number of groups obeys Poisson distribution with mean value, $\lambda$, 
and the number of particles in group has the geometrical distribution 
(with the probability $\alpha$ with at least one particle per group. 
The multiplicity probability density to have $N$ particles in interval $\Delta y$~\cite{Bogolyubsky:1994qg}:
\begin{equation}
  P(N) = \sum_{m=0}^{m=N}\frac{e^{-\lambda}\lambda^{m}}{m!}(1-\alpha)^{N-m}\alpha^m .
\end{equation}

  We may consider two cases: the characteristic width of the group is 0 (point-like group)
and all particle in group have the same $y=y_c$ (Fig.~\ref{fig:interm_groups} left) and non-point-like groups -- particles in group are distributed according Gaussian distribution 
(with $\sigma$) in the vicinity of $y_c$ (Fig.~\ref{fig:interm_groups} right).
The comparison of the $F_2$(M) behaviour for  the independent particle production and 
production of the particles in the point-like groups is shown 
in Fig.~\ref{fig:f2_vs_M} (left). 
Parameters of the Poisson and geometrical probability density functions are taken 
such that in the case of independent particle production and 
production in groups the mean multiplicity of particles in the 
interval $\Delta y$ is $\approx$100 particles/event.
\begin{figure}[H]
  \centering
  \includegraphics[width=6.5 cm]{fig1a.png}
  \includegraphics[width=6.5 cm]{fig1b.png}
  \caption{The consequent division of the interval $\Delta y$ into bins. Particles are organized in point-like groups (left) and non point-like groups (right).}
  \label{fig:interm_groups}
\end{figure}

\begin{figure}[H]
  \centering
  \includegraphics[width=9.0 cm]{F2_toy_1.png}
  \includegraphics[width=9.0 cm]{F2_toy_2.png}
  \caption{$F_2$ as a function of $M$ for point-like (left) and for non-point-like groups (right)~\cite{Cheremnova:2022fsd}.}
  \label{fig:f2_vs_M}
\end{figure}

In the case of point-like groups, $F_i(M)$ is:

\begin{equation}
F_i(M) = \sum_{k=0}^{k=i-1}A_k M^k .
\end{equation}

The evaluation of $F_{i}(M)$ function and its parameters are presented in Ref.~\cite{Bogolyubsky:1994qg}. 
For point-like groups uniformly distributed over interval: $F_2(M) = A_0+A_1*M$, where 
$A_0 = 1 - 2*(1-\alpha)(1-e^{-\lambda})/\lambda$ and 
$A_1=2*(1-\alpha)(1-e^{-\lambda})/\lambda$.

For non-point-like groups $F_i(M)$ depends also on the characteristic widths of groups. The cases with one group type ($\sigma$) and two group types with the different width ($\sigma_1>\sigma_2$) are presented in Fig.~\ref{fig:f2_vs_M} (right). 
$F_2$ grows until bin size $\delta y=\Delta M/M < \sigma$ then it starts to flatten. In the case of two groups it starts to be flat when the smallest group width is larger than the bin size. For several characteristic processes with different width ($\sigma_1>\sigma_2>…>\sigma_N$) $F_i$ is flat when $\delta y<<\sigma_N$. The power of growth inversely proportional to the mean number of groups per interval, proportional to the mean number of particles per group and depends on the widths of the characteristic processes as described in Ref.~\cite{Bogolyubsky:1994qg,Bogolyubsky:1995vr}.
   In Ref.~\cite{Cheremnova:2022fsd} it is shown how detector effects
affect the normalized factorial moments dependency: particle identification affects the particle rapidity, finite track resolution behaves as the additional group size, track reconstruction inefficiency and purity, two-tracks reconstruction inefficiency change the number of particles in group and may change the number of groups  which in turn change the power of the multiparticle correlations. These effects can be treated in a different way. To avoid influence of particle identification one moves from rapidity to pseudorapidity. Other sources of normalized factorial moments dependency change can be treated using one of the regularization methods~\cite{Cheremnova:2022fsd} with good enough accuracy.



 The possibility to distinguish the different types of the phase 
transition at $Au + Au$ collisions at $\sqrt{s_{NN}} = 7.7$ GeV
and 11.5 GeV was studied using three Monte Carlo generators, namely, UrQMD\cite{Bass:1998ca}, vHLLE+UrQMD (called further the vHLLE model)
\cite{Karpenko:2015xea} and HYDJET++\cite{Lokhtin:2008xi}. All calculations were done within the acceptance of MPD~\cite{Abraamyan:2011zz} detector. It was shown that plateau of $F_2(M)$ reaches at M$\sim$10 and the height of plateau is different depending on the collision energy for the phase transition of the 1st order while no energy dependence is observed for the crossover case~\cite{Kodolova:2021yoh}. Further studies show that the difference in energy dependence is not connected neither with collision volume, nor with cascade or multiplicity but is the characteristic of the type of phase transition and hydrodynamical phase.
Study of events fully reconstructed in detector reveals that identification inefficient affect strongly the result and we were forced to move to the pure spacial variables, i.e. pseudorapidity. It was developed unfolding procedure for the factorial moments which should be applied for each division M independently-- DEFINE M -- .
   Reconstructed and generated factorial moments of the second order
are presented in Fig.~\ref{fig:recogen} for the collision energy 7.7 GeV and 11.5 GeV. The height of plateau changes for the factorial moments calculated from reconstructed tracks with respect to the true value. Fig.~\ref{fig:recogenplateau} presents the energy dependence on the plateau height. Assuming simplest mathematical model, we may suppose that detector effects do not affect the characteristic width of clusters but change the number of clusters and the number of particles per cluster. Using unfolding procedure one can restore the dependence of the factorial moments on the size of bin and Fig.~\ref{fig:recogenplateau} shows the true and unfolded values of the plateau height. 

\begin{figure}[H]
  \centering
  \includegraphics[width=9 cm]{6.png}
  \includegraphics[width=9 cm]{7.png}
  \caption{Factorial moments of the multiplicity distribution in the pseudorapidity interval for generator and reconstructed particles for the collision energy 7.7 GeV (up) and 11.5 GeV (bottom). Black color corresponds to events with a first-order phase transition, red - with crossover.}
  \label{fig:recogen}
\end{figure}

\begin{figure}[H]
  \centering
  \includegraphics[width=9 cm]{8.png}
  \includegraphics[width=9 cm]{F2_fit_gen_unf_UrQMD_vHLLE_minidst.png}
  \caption{Factorial moments of the multiplicity distribution in the pseudorapidity interval for generator and reconstructed particles for the collision energy 7.7 GeV (left) and 11.5 GeV (right). Black color corresponds to events with a first-order phase transition, red - with crossover.}
  \label{fig:recogenplateau}
\end{figure}

